Time and Memory Trade-off of KV-Cache Compression in Tensor Transformer Decoding

The key-value (KV) cache in the tensor version of transformers presents a significant bottleneck during inference. While previous work analyzes the fundamental space complexity barriers in standard attention mechanisms [Haris and Onak, 2025], our work generalizes the space complexity barriers result to tensor attention version. Our theoretical contributions rely on a reduction from communication complexity and deduce the memory lower bound for tensor-structured attention mechanisms when $d = \Omega(\log n)$. Furthermore, we introduce two types of tensor attention cache and present a trade-off between time and memory for two scenarios. Overall, our work provides a theoretical foundation for us to understand the time-memory tradeoff of KV-Cache compression in tensor attention decoding and offers more perspectives in developing more memory-efficient tensor attention Transformer architectures.

==> 9_app_preli.tex <==
\paragraph{Roadmap.}
In Section~\ref{sec:app_preli} we provide the necessary background.
In Section~\ref{sec:more_related_work}, we present more related work.
In Section~\ref{sec:app_mem_lb}, we present our lower bound results for memory usage.


\section{Preliminary}\label{sec:app_preli}
\Yu{We need to delete Appendix~\ref{sec:app_preli} after addressed all the nametags in the main body.}

In this section, we introduce the preliminaries.
Section~\ref{sec:app_preli:columnwise_kronecker} introduces some useful definitions.
Section~\ref{sec:app_preli:attn_four} formalizes the attention mechanism with four cache matrices.
Section~\ref{sec:app_preli:attn_two} defines the attention mechanism with two cache matrices.
Section~\ref{sec:app_preli:jl_random_projection} discusses the Johnson-Linderstrauss (JL) random projection.
Section~\ref{sec:app_preli:comm_complexity} reviews the communication complexity model.
Section~\ref{sec:app_preli:index_problem} presents the \textsc{Index} problem.
Section~\ref{sec:app_preli:index_lower_bound} covers the communication complexity lower bound of the \textsc{Index} problem.


\subsection{Notations}\label{sec:app_preli:notation}

For $n \in \mathbb{Z}^+$, we use $[n]$ to denote set $\{1,2,\cdots, n\}$. We use $\E[\cdot]$ to denote the expectation.
We use $\var[\cdot]$ to represent the variance.
We use $\Pr[\cdot]$ to denote the probability.
We use $\mathbbm{1}\{C\}$ to represent an indicator variable that takes the value $1$ when condition $C$ holds and $0$ otherwise. $B^\top$ is defined as $(B^\top)_{i,j}:=B_{j,i}$. 
We use $x_{i,j}$ to denote the $j$-th coordinate of $x_i \in \R^n$.
We use $\|x\|_p$ to denote the $\ell_p$ norm of a vector $x \in \R^n$, i.e., $\|x\|_1 := \sum_{i=1}^n |x_i|$, $\|x\|_2 := (\sum_{i=1}^n x_i^2)^{1/2}$.
Suppose there are two vectors $c,d$ of the same length, we denote the entry-wise multiplication using the notation $c \odot d$; that is, the $i$-th entry in that vector is $c_i d_i$. 
We use ${\bf 0}_d$ to represent the vector of all zeros in dimension d.
We use $|M|$ to denote the length of a sequence $M$.
For two vectors $x \in \R^n$ and $y \in \R^n$, we use $\langle x, y \rangle$ to denote the inner product between $x,y$, i.e., $\langle x, y \rangle = \sum_{i=1}^n x_i y_i$.





\subsection{Attention Mechanism for Two Cache Matrices Case}\label{sec:app_preli:attn_two}
Next, we define the attention mechanism that consolidates the four KV cache matrices into two, leveraging the column-wise Kronecker product.

\begin{definition}[Tensor Attention with KV Cache, two cache matrices case]\label{def:app_attn_two_cache}
    \begin{align*}
        \mathsf{Attn}(q_i,\wt{K}_i,\wt{V}_i) := \wt{V}_i^\top \cdot \sigma_i(\wt{K}_i \cdot q_i) \in \R^d,
    \end{align*}
    where 
    \begin{align*}
        \wt{K}_i &:= K_{1,i} \oslash K_{2,i} \in \R^{i^2 \times d}\\
        \wt{V}_i &:= V_{1,i} \oslash V_{2,i} \in \R^{i^2 \times d}
    \end{align*}
\end{definition}

This definition converts the original four KV cache matrices into two matrices, $\wt{K}_i$ and $\wt{V}_i$, each of size $i^2 \times d$, by precomputing the column-wise Kronecker products. This approach reflects the trade-off between preprocessing and space complexity, as discussed in Section~\ref{sec:app_mem_lb}.



\subsection{Johnson-Linderstrauss (JL) Random Projections}\label{sec:app_preli:jl_random_projection}

In this section, we introduce a key result from random projection theory, the Johnson-Lindenstrauss (JL) Random Projection, which enables dimensionality reduction while approximately preserving inner products.

In this section, we introduce some concepts about JL-transform from~\cite{w14_book}.

\begin{definition}[Definition 3 in~\cite{w14_book}, JL-tranform]\label{def:app_jlt}
For a random matrix $S \in \R^{k \times n}$ forms a Johnson-Lindenstrauss transform with parameters $\epsilon, \delta, f$ or $\mathrm{JLT}(\epsilon, \delta, f)$ for short, if with probability at least $1 - \delta$, then for any $f$-element subset $V \subset \R^n$, for all $v,v' \in V$ it holds that
\begin{align*}
    | \langle Sv, Sv' \rangle - \langle v,v'\rangle | \leq \epsilon \|v \|_2 \| v'\|_2
\end{align*}
\end{definition}

\begin{lemma}[Theorem 4 in~\cite{w14_book}]\label{lem:app_jlt_gaussian}
If the following conditions hold:
\begin{itemize}
    \item Let $\epsilon, \delta \in (0,0.1)$.
    \item Let $S = \frac{1}{\sqrt{k}}R \in \R^{k\times n}$ where the entries $R_{i,j}$ of $R$ are independent standard normal random variables.
\end{itemize}
Then if $k = \Omega(\epsilon^{-2} \log (f/\delta))$, we have:
\begin{itemize}
    \item $S$ is a $\mathrm{JLT(\epsilon, \delta, f)}$.
\end{itemize}
\end{lemma}

\Yu{Why is this totally different to Lemma 3.5?}
\begin{lemma}[Johnson-Linderstrauss (JL) Random Projections, {\color{red}Zhao: Please cite some textbook or well-know papers}]
    \label{lem:app_inner-product-jl-for-all}
    If the following conditions hold:
    \begin{itemize}
        \item Suppose we have $n$ points $p_1,...,p_n \in \R^n$ such that $\|p_i\|_2 \leq 1$ for all $i \in [n]$.
        \item Let $f:\R^n\to \R^d$ be a random mapping defined as $f(u) = \frac{1}{\sqrt{d}}Au$ where $A \in \R^{d\times n}$ is a random matrix with its entries drawn independently from a standard normal distribution.
        \item Let $d \geq \Omega(\epsilon^{-2}\log(n))$.
    \end{itemize}
    Then with probability at least $1-\frac{1}{n}$ it holds for all $(i,j) \in [n]^2$ that:
    \begin{align*}
    |p_i^\top p_j - f(p_i)^\top f(p_j)| \leq \epsilon.
    \end{align*}
\end{lemma}
\begin{proof}
    Setting parameters $k = d$ $f = n$ and $\delta = 1/n$, by Lemma~\ref{lem:app_jlt_gaussian}, we have if $d = \Omega(\epsilon^{-2}\log(n))$, then with probability $1-\frac{1}{n}$, for all $i,j \in [n]^2$, we have
    \begin{align*}
        |p_i^\top p_j - f(p_i)^\top f(p_j)| \leq &~ \epsilon \|p_i\|_2 \|p_j\|_2 \\
        \leq &~ \epsilon
    \end{align*}
    where the first step follows from Definition~\ref{def:app_jlt}, and the second step follows from that $\|p_i\|_2 \leq 1$ for all $i \in [n]$.
\end{proof}

This lemma guarantees that a random projection into a logarithmic-dimensional space preserves pairwise inner products within an $\epsilon$-error with high probability.

\subsection{Communication Complexity}\label{sec:app_preli:comm_complexity}

In the most basic communication model~\cite{ry20}, Alice and Bob possess two $n$-bit strings, $x$ and $y$ respectively.
They wish to compute a function $f(x, y)$ by exchanging information in a certain number of rounds. 
They both have access to unlimited
computing resources, and their goal is to minimize the total amount of communication, in terms of bits, that they exchange in a fixed number of rounds.
A (potentially randomized) scheme for communicating a function $f$ is called a communication {\bf protocol}. 
The {\bf cost} of a protocol is the number of bits exchanged between Alice and Bob in the worst case.
We say that a (randomized) protocol has error $\epsilon$ if its error probability over its randomness for any input pair
$(x, y)$ is at most $\epsilon$.

\subsection{The Index Communication Problem}\label{sec:app_preli:index_problem}

Now we introduce the \textsc{Index} problem, a classic one-way communication complexity problem, whose hardness is crucial in our lower bound proofs.

\begin{definition}[]
In the \textsc{Index} problem, Alice holds a bit string $x \in \{0,1\}^n$ and Bob holds an index $i \in [n]$. Alice sends a single message (one-way) $M \in \{0,1\}^*$ to Bob, aiming to output $x_i$ with probability at least $2/3$.
\end{definition}

This definition formalizes a minimal communication setting where Alice's message must encode sufficient information for Bob to retrieve a specific bit with high probability.

\subsection{Lower Bound on the Index Problem}\label{sec:app_preli:index_lower_bound}
Here, we present a well-established result in communication complexity: the hardness of the \textsc{Index} problem under one-way, randomized protocols.

\begin{lemma}[Compelxity of the \textsc{Index} Problem, Formal Version of Lemma~\ref{lem:index_lb}, ]\label{lem:app_index_lb}
The one-way, randomized communication complexity of \textsc{Index} is $\Omega(n)$.
\end{lemma}




